The sociospatial factors of death: Analyzing effects of geospatially-distributed variables in a Bayesian mortality model for Hong Kong

Human mortality is in part a function of multiple socioeconomic factors that differ both spatially and temporally. Adjusting for other covariates, the human lifespan is positively associated with household wealth. However, the extent to which mortality in a geographical region is a function of socioeconomic factors in both that region and its neighbors is unclear. There is also little information on the temporal components of this relationship. Using the districts of Hong Kong over multiple census years as a case study, we demonstrate that there are differences in how wealth indicator variables are associated with longevity in (a) areas that are affluent but neighbored by socially deprived districts versus (b) wealthy areas surrounded by similarly wealthy districts. We also show that the inclusion of spatially-distributed variables reduces uncertainty in mortality rate predictions in each census year when compared with a baseline model. Our results suggest that geographic mortality models should incorporate nonlocal information (e.g., spatial neighbors) to lower the variance of their mortality estimates, and point to a more in-depth analysis of sociospatial spillover effects on mortality rates.

==> sections/cod.tex <==

Our initial analysis has shown an uptrend in the number of deaths caused by Pneumonia starting from 2008 as shown in Fig \ref{fig:top-five}. Upon further investigation of the dataset, we have confirmed that Pneumonia is the main driver of this unusual trend. On March 19th, 2016, a total of 35\% of the death records of that day were caused by Pneumonia as illustrated in Fig \ref{fig:main}). 

\begin{figure}[!h]
    \centering
    \includegraphics[width=\columnwidth]{oldfigures/spikes.png}
    \caption{The years highlighted in orange (2008), and green (2014, 2015, 2016) have a slightly higher average of daily death records, with 2016 being the year with the highest daily death records.}
    \label{fig:series} 
\end{figure}

\begin{figure}[!h] 
    \centering
    \includegraphics[width=\columnwidth]{oldfigures/rate.png}
    \caption{Mortality rate compared to population growth over the last few decades.} 
    \label{fig:rates}
\end{figure}

  \begin{figure}[!h]
    \centering
    \includegraphics[width=\columnwidth]{oldfigures/main.png}
    \caption{ 
    A time series of daily death records caused by Pneumonia in 2016.
    The bottom panel highlights an unusual spike on March 19th, 
    which resulted in 2016 being the year with the highest daily death records in the dataset.
    } 
    \label{fig:main} 
\end{figure}


\begin{figure*}[!ht] 
    \centering 
    \includegraphics[width=\textwidth]{oldfigures/cod.png}
    \includegraphics[width=\textwidth]{oldfigures/dcod.png}
    \caption{A closer look at the top-five cause of deaths per district.}
    \label{fig:top-five}
\end{figure*}

==> sections/future.tex <==
Future work we conduct using this dataset rests on the confluence of our (MassMutual - UVM) joint research interests and the applicability of our results to the life insurance industry more broadly. 
We envision a suite of possible non-mutually-exclusive future directions;
those of which we judge most promising we review presently:
\begin{itemize}
    \item We estimate that the lowest-hanging fruit is a statistical time series analysis of observed birth, death, and disease time series. Aside from providing a ``training ground'' of sorts for time series prediction algorithms---algorithms that are widely applicable inside a life insurance firm in general, as well as of substantial research interest in their own right---such efforts could enable a life insurance firm to better predict future birth/death ratios or trends and seasonality in causes of death, which have obvious ramifications for demand planning and future financial asset requirements.
    \item A related, but slightly more involved, analysis would take geographic variation into account. Though Hong Kong is a small island territory, it does exhibit significant inter-TPU variation in occupations, income, foreign inhabitant density, and residence status of workers, as we have reviewed above.
    Using this heterogeneity as exogenous features in a time series prediction task could lead to increased accuracy in prediction and also shed more light on the fine-grained covariance between social indicators and disease trends, for example. 
    The granularity at which the social and economic measurements have been taken, combined with a predictive time series modeling approach, could provide a baseline for research into profitable hypothetical micro-targeting of life insurance policies. 
    \item Finally, if we were able to obtain access to datasets similar to this one for a variety of countries, a multi-national cross-sectional study of the determinants of demand for life insurance, causes of death, and the interplay between them would become a possibility. 
    Although there have been many large studies of demand for life insurance in developed nations, the data used in these studies has largely been aggregated at a relatively coarse level
    \cite{zietz2003examination,li2007demand}. 
    Incorporating fine time and geographic resolution could be a significant step forward in understanding demand for life insurance and its interaction with population health measures.
\end{itemize}
